Strategic Workforce Planning in Crowdsourced Delivery with Hybrid Driver Fleets

Nowadays, logistics service providers (LSPs) increasingly consider using a crowdsourced workforce on the last mile to fulfill customers' expectations regarding same-day or on-demand delivery at reduced costs. The crowdsourced workforce's availability is, however, uncertain. Therefore, LSPs often hire additional fixed employees to perform deliveries when the availability of crowdsourced drivers is low. In this context, the reliability versus flexibility trade-off which LSPs face over a longer period, e.g., a year, remains unstudied. Against this background, we jointly study a workforce planning problem that considers fixed drivers (FDs) and the temporal development of the crowdsourced driver (CD) fleet over a long-term time horizon. We consider two types of CDs, gigworkers (GWs) and occasional drivers (ODs). While GWs are not sensitive to the request's destination and typically exhibit high availability, ODs only serve requests whose origin and destination coincide with their own private route's origin and destination. Moreover, to account for time horizon-specific dynamics, we consider stochastic turnover for both FDs and CDs as well as stochastic CD fleet growth. We formulate the resulting workforce planning problem as a Markov decision process (MDP) whose reward function reflects total costs, i.e., wages and operational costs arising from serving demand with FDs and CDs, and solve it via approximate dynamic programming (ADP). Applying our approach to an environment based on real-world demand data from GrubHub, we find that in fleets consisting of FDs and CDs, ADP-based hiring policies can outperform myopic hiring policies by up to 19% in total costs. In the studied setting, we observed that GWs reduce the LSP's total costs more than ODs. When we account for CDs' increased resignation probability when not being matched with enough requests, the amount of required FDs increases.

==> contents/Conclusions.tex <==
\section{Conclusion}
\jlmargin{
\begin{itemize}
\item Taking into account future CD supply yields cost saving potentials in terms of FD fixed costs
\item Potential depends on a number of factors: CD compensation, initial fleet compositions, mobility patterns, demand scenarios, etc.
\end{itemize}}{tbd}

==> contents/basics.tex <==
%----------------------------------------------------------------------------------
% basic commands and style changes
% author: Maximilian Schiffer
% version: 1.0 / 11.05.2017
%----------------------------------------------------------------------------------
\renewcommand{\UrlFont}{\footnotesize}
\Urlmuskip=0mu plus 4mu
% fix old math tex
\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}
\makeatother

% set pathes for graphics and pgfplots
\graphicspath{
	{./graphics/}}
\pgfplotsset{
	/pgf/number format/use comma,
	compat=1.7
}
%\usepgfplotslibrary{external}\tikzexternalize[prefix=./graphics/tikz/n]

% some changes to the normal revtex style
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\counterwithin*{equation}{section}

% Natbib setup for author-year style
\bibpunct[, ]{(}{)}{,}{a}{}{,}%
\def\bibfont{\footnotesize}%
\def\bibsep{\smallskipamount}%
\def\bibhang{24pt}%
\def\newblock{\ }%
\def\BIBand{and}%

% some nice table cell styles and commands
%\newcolumntype{Lt}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}t{#1}}
%\newcolumntype{Ct}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}t{#1}}
%\newcolumntype{Rt}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}t{#1}}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}
%\newcolumntype{Lb}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}b{#1}}
%\newcolumntype{Cb}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}b{#1}}
%\newcolumntype{Rb}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}b{#1}}

\def\VRHDW#1#2#3{\vrule height #1 depth #2 width #3}
%\newcommand{\up}{\VRHDW{1.5em}{0em}{0em}} % stretch above (for tables (8/10 makes 1em = 8pt)
%\newcommand{\down}{\VRHDW{0em}{0.625em}{0em}} % stretch below
\def\updown{\up\down}

% redefine algorithm
\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother


% set equation style
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\counterwithin*{equation}{section}


%set own font type
\newenvironment{myfont}{\fontfamily{ccr}\selectfont}{\par}
\DeclareTextFontCommand{\textmyfont}{\myfont}

% diverse
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
%\newcommand{\red}[1]{\textcolor{red}{#1}}
%\newcommand{\blue}[1]{\textcolor{blue}{#1}}

% colors
\definecolor{lightblue}{rgb}{0.60784,0.76078,0.90196}
\definecolor{darkblue}{rgb}{0.26667,0.44706,0.76863}
\definecolor{lightgreen}{rgb}{0.66275,0.81569,0.55686}
\definecolor{darkgreen}{rgb}{0.43922,0.67843,0.27843}
\definecolor{orange}{rgb}{0.92941,0.49020,0.19216}
\definecolor{yellow}{rgb}{1.00000,0.75294,0.00000}
\definecolor{grey}{rgb}{0.64706,0.64706,0.64706}
\definecolor{purple}{rgb}{0.51373,0.23529,0.04706}
\definecolor{black}{rgb}{0,0,0}
\definecolor{silver}{rgb}{0.75294,0.75294,0.79254}

% math
\newcommand{\summe}[1]{\sum_{\scriptstyle\mathclap{#1}}}

% link and color the doi
\definecolor{doicolor}{rgb}{0.12157,0.30588,0.47451}
%\def\mybibdoicolor{\color{darkblue}} %change color to suit.
%\newcommand*{\doi}[1]{doi: \href{http://dx.doi.org/#1}{\textcolor{red}{#1}}}
\newcommand*{\doi}[1]{\textcolor{doicolor}{doi:\url{#1}}}

==> resources/abbreviations.tex <==
% A

% B

% C

% D

% E

% F

% G

% H

% I

% J

% K

% L

% M

% N

% O

% P

% Q

% R

% S

% T

% U

% V

% W

% X

% Y

% Z


==> resources/commands.tex <==
%% additional user defined commands

